Adaptive Instrument Design for Indirect Experiments

Indirect experiments provide a valuable framework for estimating treatment effects in situations where conducting randomized control trials (RCTs) is impractical or unethical. Unlike RCTs, indirect experiments estimate treatment effects by leveraging (conditional) instrumental variables, enabling estimation through encouragement and recommendation rather than strict treatment assignment. However, the sample efficiency of such estimators depends not only on the inherent variability in outcomes but also on the varying compliance levels of users with the instrumental variables and the choice of estimator being used, especially when dealing with numerous instrumental variables. While adaptive experiment design has a rich literature for direct experiments, in this paper we take the initial steps towards enhancing sample efficiency for indirect experiments by adaptively designing a data collection policy over instrumental variables. Our main contribution is a practical computational procedure that utilizes influence functions to search for an optimal data collection policy, minimizing the mean-squared error of the desired (non-linear) estimator. Through experiments conducted in various domains inspired by real-world applications, we showcase how our method can significantly improve the sample efficiency of indirect experiments.

==> adaptive_instrument_design.tex <==
\section{Adaptive Instrument Design}

Discussion in Section \ref{sec:understand} highlights that the optimal design of instruments not only depends on the data-generating process (e.g., heteroskedasticity in compliances $Z|X$ and outcomes $Y$, even given a specific covariate $X$) but also on the estimators $f(\cdot; \theta)$ (e.g., weighted, (non-)linear). In this section, we provide a general gradient-based optimization procedure to find $\pi^*$ that tackles all of these problems simultaneously. 
To begin, observe that by using the REINFORCE trick \cite{williams1992simple},
\begin{align}
    \nabla \mathcal L(\pi) = \!\!\!\underset{D_n\sim \pi}{\E} \brr{\mse\br{\theta\br{D_n}} \frac{\partial \log \Pr(D_n; \pi)}{\partial \pi}} \overset{(a)}{=} \!\!\!\underset{D_n\sim \pi}{\E} \brr{\mse\br{\theta\br{D_n}} \sum_{i=1}^n  \frac{\partial \log \pi(Z_i|X_i)}{\partial \pi}} \label{eqn:reinforcee}
\end{align}
where $(a)$ follows because $\Pr(D_n;\pi)$ is the probability of observing the entire dataset $D_n$, 
\begin{align}
    \Pr(D_n; \pi) = \prod_{i=1}^n \Pr(X_i,U_i)\pi(Z_i|X_i)\Pr(A_i|X_i,  U_i, Z_i)\Pr(Y_i|X_i, U_i, A_i). 
\end{align}
Gradient in \ref{eqn:reinforcee} is appealing as it provides an unbiased direction to update $\pi$, and encapsulates properties of both the data-generating process and the estimators as a black-box in $\mse\br{\theta\br{D_n}}$.
However, as we will discuss and address in Sections \ref{sec:varred} and \ref{sec:mseshift},  gradient in \ref{eqn:reinforcee} is impractical as-is:
\begin{itemize}[leftmargin=*]
    \item \textbf{Challenge 1: }The variance of sample estimate of $\nabla \mathcal L(\pi) $ can be $\Theta (n)$, i.e., it can grow \textit{linearly} in the size of $D_n$, making the optimization process prohibitively inefficient.
    \item \textbf{Challenge 2: } Optimization using \ref{eqn:reinforcee} would require evaluating $\nabla \mathcal L(\pi)$ for a $\pi$ different from $\pi'$ that was used to collect the data.  If off-policy correction is done using  importance weighting \citep{precup2000eligibility}, then the variance can be $\mathcal O(\rho_{\max}^n)$, i.e., blow \textit{exponentially} with $n$. \ycinline{Use lower bound here or Have an example to show that upper bound is tight?} 
\end{itemize}


 \begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{images/grad_var_mis.pdf}
    \includegraphics[width=0.3\textwidth]{images/sampler_var.pdf}
    \caption{\textbf{(Left)}  Challenge 1: Variance of different gradient estimators when the function approximator is \textit{mis-specified}.  \textbf{(Right)} Challenge 2: Variance in estimating $\mse$ of an IV estimator using different samplers. Online and rejection sampling curves are overlapping. \ycinline{update plots}} 
    \label{fig:gradvar}
\end{figure}

\subsection{Efficient Variance Reduction of Gradient Estimates }
\label{sec:varred}
To illustrate Challenge 1, let $\hat \nabla \mathcal L(\pi)$ be the estimate obtained using a single $D_n$ sample,
\begin{align}
    \hat \nabla \mathcal L(\pi) \coloneqq \mse\br{\theta\br{D_n}} \sum_{i=1}^n  \frac{\partial \log \pi(Z_i|X_i)}{\partial \pi} \label{eqn:samplereinforce}.
\end{align}
Intuitively, as the `reward' $\mse\br{\theta\br{D_n}}$ associated with all the decisions $\{\pi(Z_i|X_i)\}_{i=1}^n$ is the same, credit assignment becomes difficult and thus identifying useful decisions becomes harder as $n$ increases. We formalize this intuition in the following (proofs are deferred to Appendix \ref{apx:sec:biasvar}).
\begin{prop}[Informal]
\thlabel{prop:naive}
    If $\mse(\theta(D_n))$ is leave-one-out stable and $n \|\mse\br{\theta(D_n)}\|_{L^2}^2=\Omega(\alpha(n))=\omega(1)$, we have $\var(\hat \nabla \mathcal L(\pi))=\Omega(\alpha(n))$.
\end{prop}
 \begin{rem}
     In many cases, we would expect that the mean squared error decays at the rate of $n^{-1/2}$ (unless we can invoke a fast parametric rate of $1/n$, which holds under strong convexity assumptions); in such cases, we have that $\alpha(n)=\omega(1)$ and $\var(\hat \nabla \mathcal L(\pi))$ can grow with the sample size. Moreover, if the mean squared error does not converge to zero, due to persistent approximation error, or local optima in the optimization, or if \ref{eqn:inv} is ill-posed when dealing with non-parametric estimators, then the variance can grow linearly, i.e. $\alpha(n)=\Theta(n)$. See Figure \ref{fig:gradvar}.
 \end{rem}
\paragraph{Control variates:} One approach for variance reduction is to use control variates \citep{greensmith2004variance} that are independent of the decisions, i.e., $\{\pi(Z_i|X_i)\}_{i=1}^n$. However, as each decision $\pi(Z_i|X_i)$ is independent of the other $\pi(Z_j|X_j)$, we can leverage this factorization to design control variates for each decision  $\pi(Z_i|X_i)$ that depends on all other decisions $\{\pi(Z_j|X_j)\}_{j\neq i}$, but itself. To observe this, let $D_{n\backslash i}$ be the entire dataset albeit the $i^\text{th}$ data tuple $S_i$, then, 
\begin{align}
\small  
    \!\!\!\underset{{D_n\sim\pi}}{\E}\brr{ \mse\br{\theta\br{D_{n\backslash i}}}\frac{\partial \log \pi(Z_i|X_i)}{\partial \pi} }\!\! = \!\!\! \underset{{D_{n\backslash i}\sim\pi}}{\E}\brr{\mse\br{\theta\br{D_{n\backslash i}}} \!\underset{ S_i\sim\pi}{\E}\brr{\frac{\partial \log \pi(Z_i|X_i)}{\partial \pi} }} \!\!= 0. \label{eqn:cv0}
\end{align}
This insight combines the ideas in RL for action-factorized baselines \citep{wu2018variance,liu2017action} with leave-one-out control variates \citep{kool2019buy,salimans2014using,richter2020vargrad,titsias2022double,shi2022gradient}.
Combining \ref{eqn:samplereinforce} with the insight in \ref{eqn:cv0}, the gradient estimate $ {\hat \nabla}^\texttt{CV} \mathcal L(\pi)$ in \ref{eqn:samplereinforcecv} can be shown to drastically reduce the variance, while still being unbiased,
\begin{align}
     {\hat \nabla}^\texttt{CV} \mathcal L(\pi) \coloneqq \sum_{i=1}^n  \frac{\partial \log \pi(Z_i|X_i)}{\partial \pi} \br{\mse\br{\theta\br{D_n}} - \mse\br{\theta\br{D_{n\backslash i}}} }. \label{eqn:samplereinforcecv}
\end{align}
\begin{prop}[Informal]
\thlabel{prop:cv}
   $\E [{\hat \nabla}^\texttt{CV} \mathcal L(\pi)] = \nabla \mathcal L(\pi)$. Further, if $\mse(\theta(D_n))$ is leave-one-out stable then $\var({\hat \nabla}^\texttt{CV} \mathcal L(\pi)) = \mathcal O(1) $.
\end{prop}
 \begin{rem}
  Unlike \thref{prop:naive}, \thref{prop:cv} holds irrespective of $\alpha(n)$, thus provides a more reliable gradient estimator even if the function approximator is mis-specified, or optimization is susceptible to local optima, or if \ref{eqn:inv} is ill-posed when dealing with non-parametric estimators.
 \end{rem}
\textbf{Influence functions:} Using control variates was beneficial as $  {\hat \nabla}^\texttt{CV} \mathcal L(\pi) $ provided variance reduction compared to $  {\hat \nabla} \mathcal L(\pi) $. However, observe that computation required for estimating $  {\hat \nabla}^\texttt{CV} \mathcal L(\pi) $ can still be prohibitively expensive as for \textit{each}  $\nabla \log \pi(Z_i|X_i)$ in \ref{eqn:samplereinforcecv}, an entire separate optimization process is required for explicit re-training to estimate the control variate $\mse(\theta(D_{n\backslash i})) $. This computational inefficiency is exacerbated when $n$ is large. In contrast, recall from \ref{eqn:samplereinforce} that  $  {\hat \nabla} \mathcal L(\pi) $ only required estimating $\mse(\theta(D_{n})) $ \textit{once}, independent of $n$. 

To be efficient in terms of \textit{both} the variance and the computation, we propose estimating $\mse\br{\theta\br{D_n}} - \mse\br{\theta\br{D_{n\backslash i}}} $ using influence functions \citep{cook1982residuals,fisher2021visually}. As we discuss below, this requires only a \textit{single} optimization process for estimating $\mse\br{\theta\br{D_n}} - \mse(\theta(D_{n\backslash i})) $ for every $i$, and thus preserves the best of both $  {\hat \nabla}^\texttt{CV} \mathcal L(\pi) $ and $  {\hat \nabla} \mathcal L(\pi) $. 

Let $\mathbb D$ be the distribution function induced by the dataset $D_n$, and with a slight overload of notation, we let $\theta(D_n) \equiv \theta(\mathbb D)$.
Perturbing the i-th training sample $S_i$  is equivalent to perturbing $\mathbb D$ to create a new distribution $\mathbb D_{i,\epsilon} \coloneqq (1- \epsilon) \mathbb D + \epsilon \delta(S_i)$, where $\delta(S_i)$ denotes the Dirac distribution on the  sample $S_i$.
For $\epsilon=-1/n$, observe that $\mathbb D_{i,\epsilon}$ corresponds to the distribution function without the sample $S_i$, i.e., distribution induced by $D_{n\backslash i}$.
From this perspective, $\mse(\theta(\cdot))$ corresponds to a \textit{functional} of the data distribution function $\mathbb D$, and thus Von Mises expansion  \citep{fernholz2012mises}, i.e., a distributional analog of the Taylor expansion for statistical functionals, 
to directly approximate $\mse(\theta(\mathbb D_{i,\epsilon}))$ in terms of $\mse(\theta(\mathbb D))$ as \ycinline{Defer discussion of seed to appendix}
\begin{align}
    \mse\br{\theta(\mathbb D_{i,\epsilon})} = \mse\br{\theta\br{\mathbb D}} + \sum_{k=1}^\infty \frac{\epsilon^k}{k!} \,  \mathcal I^{(k)}_\mse(S_i), \label{eqn:LOOmain}
    \\
    \text{where, }\quad  \mathcal I_\mse^{(1)}(S_i)\coloneqq \frac{\mathrm d}{\mathrm d t}\mse\Big(\theta\Big((1-t)\mathbb D + t \delta(S_i)\Big)\Big) \Big|_{t=0}
\end{align}
is the $k$-th order \textit{influence function} that operationalizes the concept of derivative for the functional $\mse(\theta(\cdot))$. That is, it characterizes the effect on $\mse$ when the training sample $S_i$ is infinitesimaly up-weighted during optimization.
Therefore, when all the higher order influence function exists, we can use \ref{eqn:LOOmain} to recover an estimate of $ \mse(\theta(D_n)) - \mse(\theta(D_{n\backslash i}))$ without re-training.
Similar conditions have also been used by prior works in the context of uncertainty quantification \citep{alaa2020discriminative}, model selection \citep{alaa2019validating}, and dataset distillation \citep{loo2023dataset}.
In practice, approximating with a $K$-th order expansion often suffices.
This permits an alternate gradient estimator $ {\hat \nabla}^\texttt{IF} \mathcal L(\pi)$ that avoids any re-computation of the mean-square-error,  and also provides adequate trade-off between variance and the bias resulting from $K$-th order approximation of \ref{eqn:LOOmain}, 
\begin{align}
     {\hat \nabla}^\texttt{IF} \mathcal L(\pi) &\coloneqq \sum_{i=1}^n  \frac{\partial \log \pi(Z_i|X_i)}{\partial \pi}  \mathcal I_\mse(S_i), &\text{where,   } \,\, \mathcal I_\mse(S_i) &\coloneqq  - \sum_{k=1}^K \frac{\epsilon^k}{k!} \,  \mathcal I^{(k)}_\mse(S_i).    \label{eqn:samplereinforceiv} 
\end{align}
\begin{prop}[Informal] If the Von-Mises expansion in \ref{eqn:LOOmain} is convergent, 
   $\E [{\hat \nabla}^\texttt{IF} \mathcal L(\pi)] = \nabla \mathcal L(\pi) + \mathcal O(n^{-K})$.  Further, if $\mse(\theta(D_n))$ is leave-one-out stable then $\var({\hat \nabla}^\texttt{IF} \mathcal L(\pi)) = \mathcal O(1)$.
\end{prop}
As the bias in the gradient is of the order $n^{-K}$, bias can be neglected even when using $K=1$.
In \thref{thm:inf} we characterize the form for $\mathcal I^{(1)}_\mse(S_i)$.
\thref{thm:inf} generalizes the influence function for standard machine learning estimators (e.g., least-sqaures, classification) \citep{koh2017understanding} to more general estimators (e.g., IV estimator, GMM estimators, double machine-learning estimators) that involve estimation of nuisance parameters $\phi$ alongside the parameters of interest $\theta$, as discussed in \ref{eqn:moments}. Since \thref{thm:inf} provides a black-box procedure, it can be used with differentiable function approximators and thus could be of independent interest.
\begin{thm}[Influence Functions for Black-box Double Estimators] If the inverses exist,
\begin{align}
   \mathcal I^{(1)}_\mse(S_i) &=   
    \frac{\mathrm d }{\mathrm d\theta} \mse(\hat \theta)\, \mathcal I^{(1)}_\theta(S_i)  \label{eqn:inff1}
    \\
     \mathcal I^{(1)}_\theta(S_i) &= - \frac{\partial M_n}{\partial \theta}^{-1}\!\!\!\!\!\!{(\hat \theta, \hat \phi)} \brr{m(S_i, \hat \theta, \hat \phi) - { \frac{\partial M_n}{\partial \phi}{(\hat \theta, \hat \phi)}\brr{\frac{\partial Q_n}{\partial \phi}^{-1}\!\!\!\!\!\!{(\hat \phi)} q(S_i, \hat \phi)}}}. \label{eqn:inff2}
\end{align}
\thlabel{thm:inf}
\end{thm}
While \ref{eqn:inff2} might look intractable at first, in Appendix \ref{apx:sec:influence} we discuss how  $\mathcal I^{(1)}_\theta(S_i)$ can be computed efficiently, without ever explicitly storing or inverting derivatives of $M_n$ or $Q_n$, using Hessian-vector products \citep{pearlmutter1994fast} readily available in auto-diff packages \citep{jax2018github,pytorch}. 
These tricks are inspired by techniques used to scale implicit gradients and influence function computation to models with millions \citep{lorraine2020optimizing} and billions \citep{grosse2023studying} of parameters.
In Appendix \ref{apx:sec:influence}, we also discuss how $ \mathcal I^{(1)}_\theta(S_i)$ can be re-used to partially estimate $\mathcal I^{(2)}_\mse(S_i)$. 
thereby making $\mathcal I_\mse(S_i)$ more accurate.
\subsection{Variance Reduced Distribution Correction}
\label{sec:mseshift}
Recall from Challenge 2 that gradient based search of $\pi^*$ would require evaluating gradient at $\pi'$ using data collected from $\pi \neq \pi'$.
A common technique in RL to address this is by using importance sampling \citep{precup2000eligibility,thomas2015safe}.
Unfortunately, as we discuss in Appendix \ref{apx:sec:rejection}, using importance sampling can blow the variance of gradient estimates \textit{exponentially} in the number of samples $n$.

\textbf{Rejection Sampling: }  Unlike RL, in our setting, the estimator $\theta(D_n)$ can be considered symmetric and thus the order of samples in $D_n$ do not matter.
Further, it may be reasonable to assume that policy ordering is robust to the dataset size, i.e., ${\E}_\pi\brr{ \mse(\theta(D_n))} \geq  {\E}_{\pi'}\brr{ \mse(\theta(D_n))}$ implies that $ {\E}_\pi\brr{ \mse(\theta(D_k))} \geq  {\E}_{\pi'}\brr{ \mse(\theta(D_k))}$, where $k<n$.
Therefore, we can combine these two insights to evaluate policies on random \textit{subsets} $D_k \subset D_n$.

Specifically, we propose using 
rejection sampling to sample data $D_k$ counter-factually, i.e., data that would have been sampled if $\pi'$ was used to collect the data, instead of $\pi$.  
For ${\mathcal L}(\pi')$, a data sample $S_i$ is accepted using the following condition
\begin{align}
    S_i = \begin{cases}
        \text{Accept} & \text{if} \quad \xi_i \leq \rho(S_i)/\rho_{\max}
        \\
        \text{Reject} & \text{Otherwise.} \label{eqn:reject}
    \end{cases}
\end{align}
where $\xi_i \sim \texttt{Uniform}(0,1)$, $\rho_{\max} \coloneqq \max_{s} \rho(s)$, and $\rho(S)$ is the importance ratio associated with a sample $S$, 
\begin{align}
\rho(S_i) \coloneqq 
\frac{\Pr(X_i,U_i)\pi'(Z_i|X_i)\Pr(A_i|Z_i,X_i,U_i)\Pr(Y_i|X_i,A_i,U_i)}{\Pr(X_i,U_i)\pi_i(Z_i|X_i)\Pr(A_i|Z_i,X_i,U_i)\Pr(Y_i|X_i,A_i,U_i)}
= \frac{\pi'(Z_i|X_i)}{\pi_i(Z_i|X_i)}.
\end{align}
Importantly, observe that \ref{eqn:reject} allows simulating samples from the data distribution governed by $\pi'$, without requiring any knowledge of the unobserved confounders $U_i$.
Further, as we have access to both $\pi'$ and $\pi_i(Z_i|X_i)$,  $\rho(S_i)$ can be obtained trivially. 
Subsequently, a random sub-set of size $k$ from the accepted samples can be then used as $D_k$.
Let $\mse^\texttt{RS}_k $ be the estimate of $\mse$ for a dataset of size $k$, obtained using rejection sampling.
Leveraging the structure in our problem, rejection sampling can drastically reduce variance compared to exponential variance from importance sampling. 
Further, it can also be shown that if $k=o(n)$, then the probability of the failure case, where the expected number of samples $n^{RS}$ accepted by rejection sampling is less than the desired $k$ samples, \textit{decays} \textit{exponentially}. 
\begin{prop}  If $k \|\mse\br{\theta(D_k)}\|_{L^2}^2=\mathcal O(\alpha(k))$ then 
   $\var\br{\mse^\texttt{RS}_k} = \mathcal O(\alpha(k)\rho_{\max}/n)$. Further, If $k=o(n)$, then
     $\Pr(n^{RS}<k) = \mathcal O(c^n)$, where $c \in [0, 1)$.  
\end{prop}

\textbf{Multi-Rejection Sampling: } While rejection sampling already provides drastic gains over importance sampling for our problem, its validity still hinges upon the support assumption which necessitates $\pi_i(Z_i|X_i) >0$ if $\pi'(Z_i|X_i)>0$ for all $i \in \{1,...,n\}$.  
This may restrict the class of policies that can be deployed, as even if $Z_i$ is not a useful instrument to sample, assigning $\pi_i(Z_i|X_i)$  to zero may be counter-productive if the collected samples are to be re-used later for rejection sampling again.
To remedy this issue, we propose the following \textit{multi}-rejection sampling strategy that is well-suited for our data collection strategy.
\begin{align}
    S_i &= \begin{cases}
        \text{Accept} & \text{if} \quad \xi_i \leq \bar \rho(S_i)/\bar \rho_{\max}
        \\
        \text{Reject} & \text{Otherwise.} \label{eqn:rejectt}
    \end{cases}
    &  \bar \rho(S_i) \coloneqq \frac{\pi'(Z_i|X_i)}{\frac{1}{n}\sum_j \pi_j(Z_i|X_i)} \label{eqn:multirss}
\end{align}
where $\bar \rho_{\max} = \max_s \bar \rho(s)$. This relaxes the support assumption enforced for every $\pi_i$ to support assumption over the \textit{union} of supports of $\{\pi_i\}_{i=1}^n$. This is crucial because if we have some initial data collected using uniform policy, then subsequent policies can be arbitrarily deterministic and the multi-rejection procedure can still use all the data and remain valid. Further, it can also be shown that the expected number of samples $n^{\text{MRS}}$ accepted under multi-rejection will always be more than or equal than using vanilla rejection sampling, irrespective of $\{\pi_i\}_{i=1}^n$.
Let $p(s)$ correspond to the probability of observing sample $s$ when using multi-rejection sampler defined in \ref{eqn:multirss},
\begin{prop} If $\forall z, x$,  $\pi'(z|x)>0$ implies $\sum_j \pi_j(z|x) > 0$, then 
$p(s) \propto \Pr(S_i=s;\pi') $ and $n^{MRS} \geq n^{RS}$.    
\end{prop}




